Brittle Minds, Fixable Activations: Understanding Belief Representations in Language Models

Despite growing interest in Theory of Mind (ToM) tasks for evaluating language models (LMs), little is known about how LMs internally represent mental states of self and others. Understanding these internal mechanisms is critical - not only to move beyond surface-level performance, but also for model alignment and safety, where subtle misattributions of mental states may go undetected in generated outputs. In this work, we present the first systematic investigation of belief representations in LMs by probing models across different scales, training regimens, and prompts - using control tasks to rule out confounds. Our experiments provide evidence that both model size and fine-tuning substantially improve LMs' internal representations of others' beliefs, which are structured - not mere by-products of spurious correlations - yet brittle to prompt variations. Crucially, we show that these representations can be strengthened: targeted edits to model activations can correct wrong ToM inferences.

==> sections/table.tex <==
\begin{table*}[t]
    \centering
    \small{
    \begin{tabular}{lllllllllll} 
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Forward Belief}} & \multicolumn{3}{c}{\textbf{Forward Action}} & \multicolumn{3}{c}{\textbf{Backward Belief}} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} 
        & & TB & FB & Both & TB & FB & Both & TB & FB & Both \\ 
        \midrule
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Llama-2-7b} & No int. & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ \\
        & ITI & $44_{+0}$ & $44_{+0}$ & $44_{+0}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $66_{\textcolor{PineGreen}{+22}}^*$ & $71_{\textcolor{PineGreen}{+27}}^*$ & $54_{\textcolor{PineGreen}{+10}}$ & $66_{\textcolor{PineGreen}{+22}}^*$ & $57_{\textcolor{PineGreen}{+13}}^*$ & $54_{\textcolor{PineGreen}{+10}}$ & $60_{\textcolor{PineGreen}{+16}}^*$ & $74_{\textcolor{PineGreen}{+30}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Llama-2-7b-chat} & No int. & $56$ & $56$ & $55$ & $69$ & $55$ & $37$ & $56$ & $56$ & $55$ \\
        & ITI & $58_{\textcolor{PineGreen}{+2}}$ & $58_{\textcolor{PineGreen}{+2}}$ & $57_{\textcolor{PineGreen}{+2}}$ & $69_{+0}$ & $55_{+0}$ & $37_{+0}$ & $58_{\textcolor{PineGreen}{+2}}$ & $60_{\textcolor{PineGreen}{+3}}$ & $57_{\textcolor{PineGreen}{+2}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $70_{\textcolor{PineGreen}{+14}}$ & $72_{\textcolor{PineGreen}{+16}}^*$ & $57_{\textcolor{PineGreen}{+2}}$ & $69_{+0}$ & $67_{\textcolor{PineGreen}{+12}}$ & $53_{\textcolor{PineGreen}{+16}}$ & $66_{\textcolor{PineGreen}{+10}}$ & $84_{\textcolor{PineGreen}{+27}}^*$ & $57_{\textcolor{PineGreen}{+2}}^*$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Llama-2-13b} & No int. & $52$ & $44$ & $35$ & $59$ & $50$ & $37$ & $46$ & $49$ & $33$ \\
        & ITI & $52_{+0}$ & $45_{\textcolor{PineGreen}{+1}}$ & $35_{+0}$ & $64_{\textcolor{PineGreen}{+5}}$ & $61_{\textcolor{PineGreen}{+11}}$ & $46_{\textcolor{PineGreen}{+9}}$ & $48_{\textcolor{PineGreen}{+2}}$ & $59_{\textcolor{PineGreen}{+10}}$ & $42_{\textcolor{PineGreen}{+9}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $85_{\textcolor{PineGreen}{+33}}^*$ & $88_{\textcolor{PineGreen}{+44}}^*$ & $66_{\textcolor{PineGreen}{+31}}^*$ & $71_{\textcolor{PineGreen}{+12}}^*$ & $69_{\textcolor{PineGreen}{+19}}^*$ & $55_{\textcolor{PineGreen}{+18}}^*$ & $75_{\textcolor{PineGreen}{+29}}^*$ & $92_{\textcolor{PineGreen}{+43}}^*$ & $59_{\textcolor{PineGreen}{+26}}^*$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Llama-2-13b-chat} & No int. & $84$ & $56$ & $47$ & $78$ & $51$ & $38$ & $72$ & $48$ & $31$ \\
        & ITI & $84_{+0}$ & $65_{\textcolor{PineGreen}{+9}}$ & $59_{\textcolor{PineGreen}{+12}}$ & $78_{+0}$ & $58_{\textcolor{PineGreen}{+7}}$ & $47_{\textcolor{PineGreen}{+9}}^*$ & $72_{+0}$ & $60_{\textcolor{PineGreen}{+12}}$ & $48_{\textcolor{PineGreen}{+17}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $97_{\textcolor{PineGreen}{+13}}^*$ & $94_{\textcolor{PineGreen}{+38}}^*$ & $91_{\textcolor{PineGreen}{+44}}^*$ & $80_{\textcolor{PineGreen}{+2}}^*$ & $71_{\textcolor{PineGreen}{+20}}^*$ & $54_{\textcolor{PineGreen}{+16}}^*$ & $97_{\textcolor{PineGreen}{+25}}$ & $94_{\textcolor{PineGreen}{+46}}^*$ & $87_{\textcolor{PineGreen}{+56}}^*$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Llama-2-70b} & No int. & $90$ & $87$ & $78$ & $93$ & $52$ & $48$ & $73$ & $53$ & $32$ \\
        & ITI & $90_{+0}$ & $90_{\textcolor{PineGreen}{+3}}$ & $78_{+0}$ & $94_{\textcolor{PineGreen}{+1}}$ & $55_{\textcolor{PineGreen}{+3}}$ & $50_{\textcolor{PineGreen}{+2}}$ & $77_{\textcolor{PineGreen}{+4}}$ & $58_{\textcolor{PineGreen}{+5}}$ & $37_{\textcolor{PineGreen}{+5}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $99_{\textcolor{PineGreen}{+9}}^*$ & $97_{\textcolor{PineGreen}{+10}}^*$ & $95_{\textcolor{PineGreen}{+17}}^*$ & $94_{\textcolor{PineGreen}{+1}}^*$ & $80_{\textcolor{PineGreen}{+28}}^*$ & $73_{\textcolor{PineGreen}{+25}}^*$ & $94_{\textcolor{PineGreen}{+21}}$ & $92_{\textcolor{PineGreen}{+39}}^*$ & $83_{\textcolor{PineGreen}{+51}}^*$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Llama-2-70b-chat} & No int. & $69$ & $75$ & $56$ & $86$ & $56$ & $52$ & $63$ & $59$ & $52$ \\
        & ITI & $69_{+0}$ & $76_{\textcolor{PineGreen}{+1}}$ & $59_{\textcolor{PineGreen}{+2}}$ & $86_{+0}$ & $56_{+0}$ & $52_{+0}$ & $63_{+0}$ & $60_{\textcolor{PineGreen}{+1}}$ & $54_{\textcolor{PineGreen}{+2}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $92_{\textcolor{PineGreen}{+23}}^*$ & $97_{\textcolor{PineGreen}{+22}}^*$ & $89_{\textcolor{PineGreen}{+32}}^*$ & $87_{\textcolor{PineGreen}{+1}}^*$ & $75_{\textcolor{PineGreen}{+19}}^*$ & $60_{\textcolor{PineGreen}{+8}}^*$ & $88_{\textcolor{PineGreen}{+25}}$ & $92_{\textcolor{PineGreen}{+33}}^*$ & $80_{\textcolor{PineGreen}{+28}}$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        \midrule
        \multirow[t]{3}{*}{Pythia-70m} & No int. & $41$ & $41$ & $37$ & $46$ & $45$ & $41$ & $44$ & $41$ & $37$ \\
        & ITI & $54_{\textcolor{PineGreen}{+13}}$ & $54_{\textcolor{PineGreen}{+13}}$ & $54_{\textcolor{PineGreen}{+17}}^*$ & $54_{\textcolor{PineGreen}{+8}}$ & $54_{\textcolor{PineGreen}{+9}}$ & $54_{\textcolor{PineGreen}{+13}}^*$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+13}}$ & $54_{\textcolor{PineGreen}{+17}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $62_{\textcolor{PineGreen}{+21}}^*$ & $56_{\textcolor{PineGreen}{+15}}^*$ & $54_{\textcolor{PineGreen}{+17}}^*$ & $59_{\textcolor{PineGreen}{+13}}^*$ & $60_{\textcolor{PineGreen}{+15}}^*$ & $58_{\textcolor{PineGreen}{+17}}^*$ & $63_{\textcolor{PineGreen}{+19}}$ & $56_{\textcolor{PineGreen}{+15}}^*$ & $54_{\textcolor{PineGreen}{+17}}^*$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Pythia-410m} & No int. & $48$ & $45$ & $45$ & $44$ & $44$ & $44$ & $44$ & $47$ & $44$ \\
        & ITI & $55_{\textcolor{PineGreen}{+7}}$ & $62_{\textcolor{PineGreen}{+17}}^*$ & $52_{\textcolor{PineGreen}{+7}}$ & $54_{\textcolor{PineGreen}{+10}}^*$ & $54_{\textcolor{PineGreen}{+10}}^*$ & $54_{\textcolor{PineGreen}{+10}}$ & $60_{\textcolor{PineGreen}{+16}}$ & $63_{\textcolor{PineGreen}{+16}}$ & $56_{\textcolor{PineGreen}{+12}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $67_{\textcolor{PineGreen}{+19}}^*$ & $64_{\textcolor{PineGreen}{+19}}^*$ & $61_{\textcolor{PineGreen}{+16}}^*$ & $56_{\textcolor{PineGreen}{+12}}^*$ & $63_{\textcolor{PineGreen}{+19}}^*$ & $56_{\textcolor{PineGreen}{+12}}^*$ & $69_{\textcolor{PineGreen}{+25}}$ & $63_{\textcolor{PineGreen}{+16}}^*$ & $60_{\textcolor{PineGreen}{+16}}$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Pythia-1b} & No int. & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ \\
        & ITI & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $59_{\textcolor{PineGreen}{+15}}^*$ & $62_{\textcolor{PineGreen}{+18}}^*$ & $54_{\textcolor{PineGreen}{+10}}$ & $57_{\textcolor{PineGreen}{+13}}$ & $59_{\textcolor{PineGreen}{+15}}$ & $56_{\textcolor{PineGreen}{+12}}$ & $57_{\textcolor{PineGreen}{+13}}$ & $60_{\textcolor{PineGreen}{+16}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Pythia-6.9b} & No int. & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ \\
        & ITI & $45_{\textcolor{PineGreen}{+1}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $44_{+0}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $56_{\textcolor{PineGreen}{+12}}$ & $71_{\textcolor{PineGreen}{+27}}^*$ & $55_{\textcolor{PineGreen}{+11}}$ & $55_{\textcolor{PineGreen}{+11}}$ & $63_{\textcolor{PineGreen}{+19}}$ & $55_{\textcolor{PineGreen}{+11}}$ & $55_{\textcolor{PineGreen}{+11}}$ & $71_{\textcolor{PineGreen}{+27}}^*$ & $55_{\textcolor{PineGreen}{+11}}$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Pythia-6.9b-chat} & No int. & $55$ & $54$ & $28$ & $36$ & $64$ & $20$ & $44$ & $67$ & $30$ \\
        & ITI & $57_{\textcolor{PineGreen}{+2}}$ & $54_{+0}$ & $28_{+0}$ & $44_{\textcolor{PineGreen}{+8}}$ & $71_{\textcolor{PineGreen}{+7}}$ & $32_{\textcolor{PineGreen}{+12}}$ & $44_{+0}$ & $67_{+0}$ & $30_{+0}^*$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $68_{\textcolor{PineGreen}{+13}}$ & $65_{\textcolor{PineGreen}{+11}}$ & $57_{\textcolor{PineGreen}{+29}}^*$ & $54_{\textcolor{PineGreen}{+18}}$ & $75_{\textcolor{PineGreen}{+11}}$ & $48_{\textcolor{PineGreen}{+28}}^*$ & $58_{\textcolor{PineGreen}{+14}}^*$ & $67_{+0}$ & $54_{\textcolor{PineGreen}{+24}}^*$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Pythia-12b} & No int. & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ \\
        & ITI & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $54_{\textcolor{PineGreen}{+10}}$ & $64_{\textcolor{PineGreen}{+20}}^*$ & $54_{\textcolor{PineGreen}{+10}}$ & $60_{\textcolor{PineGreen}{+16}}$ & $58_{\textcolor{PineGreen}{+14}}$ & $55_{\textcolor{PineGreen}{+11}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $67_{\textcolor{PineGreen}{+23}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \bottomrule
    \end{tabular}
    }
    \caption{Comparison of the effects of ITI \citep{li2023inferencetime} and CAA \citep{rimsky2023steering} activation editing methods on three tasks from BigToM \citep{gandhi2024understanding}. TB denotes a true belief task, whereas FB denotes a false belief task. The numbers represent accuracy scores, with the difference in performance compared to no intervention (No int.) indicated as subscripts (ITI $-$ No int. and CAA $-$ No int.). An asterisk ($*$) denotes a statistically significant difference from No int.\ based on a
    t-test with $p < 0.05$.}
    \label{tab:caa_results}
\end{table*}


==> sections/table_pythia_only.tex <==
\begin{table*}[t]
    \centering
    \small{
    \begin{tabular}{lllllllllll} 
        \toprule
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Forward Belief}} & \multicolumn{3}{c}{\textbf{Forward Action}} & \multicolumn{3}{c}{\textbf{Backward Belief}} \\
        \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} 
        & & TB & FB & Both & TB & FB & Both & TB & FB & Both \\ 
        \midrule
        \multirow[t]{3}{*}{Pythia-70m} & No int. & $41$ & $41$ & $37$ & $46$ & $45$ & $41$ & $44$ & $41$ & $37$ \\
        & ITI & $54_{\textcolor{PineGreen}{+13}}$ & $54_{\textcolor{PineGreen}{+13}}$ & $54_{\textcolor{PineGreen}{+17}}^*$ & $54_{\textcolor{PineGreen}{+8}}$ & $54_{\textcolor{PineGreen}{+9}}$ & $54_{\textcolor{PineGreen}{+13}}^*$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+13}}$ & $54_{\textcolor{PineGreen}{+17}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $62_{\textcolor{PineGreen}{+21}}^*$ & $56_{\textcolor{PineGreen}{+15}}^*$ & $54_{\textcolor{PineGreen}{+17}}^*$ & $59_{\textcolor{PineGreen}{+13}}^*$ & $60_{\textcolor{PineGreen}{+15}}^*$ & $58_{\textcolor{PineGreen}{+17}}^*$ & $63_{\textcolor{PineGreen}{+19}}$ & $56_{\textcolor{PineGreen}{+15}}^*$ & $54_{\textcolor{PineGreen}{+17}}^*$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Pythia-410m} & No int. & $48$ & $45$ & $45$ & $44$ & $44$ & $44$ & $44$ & $47$ & $44$ \\
        & ITI & $55_{\textcolor{PineGreen}{+7}}$ & $62_{\textcolor{PineGreen}{+17}}^*$ & $52_{\textcolor{PineGreen}{+7}}$ & $54_{\textcolor{PineGreen}{+10}}^*$ & $54_{\textcolor{PineGreen}{+10}}^*$ & $54_{\textcolor{PineGreen}{+10}}$ & $60_{\textcolor{PineGreen}{+16}}$ & $63_{\textcolor{PineGreen}{+16}}$ & $56_{\textcolor{PineGreen}{+12}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $67_{\textcolor{PineGreen}{+19}}^*$ & $64_{\textcolor{PineGreen}{+19}}^*$ & $61_{\textcolor{PineGreen}{+16}}^*$ & $56_{\textcolor{PineGreen}{+12}}^*$ & $63_{\textcolor{PineGreen}{+19}}^*$ & $56_{\textcolor{PineGreen}{+12}}^*$ & $69_{\textcolor{PineGreen}{+25}}$ & $63_{\textcolor{PineGreen}{+16}}^*$ & $60_{\textcolor{PineGreen}{+16}}$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Pythia-1b} & No int. & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ \\
        & ITI & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $59_{\textcolor{PineGreen}{+15}}^*$ & $62_{\textcolor{PineGreen}{+18}}^*$ & $54_{\textcolor{PineGreen}{+10}}$ & $57_{\textcolor{PineGreen}{+13}}$ & $59_{\textcolor{PineGreen}{+15}}$ & $56_{\textcolor{PineGreen}{+12}}$ & $57_{\textcolor{PineGreen}{+13}}$ & $60_{\textcolor{PineGreen}{+16}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Pythia-6.9b} & No int. & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ \\
        & ITI & $45_{\textcolor{PineGreen}{+1}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $44_{+0}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $56_{\textcolor{PineGreen}{+12}}$ & $71_{\textcolor{PineGreen}{+27}}^*$ & $55_{\textcolor{PineGreen}{+11}}$ & $55_{\textcolor{PineGreen}{+11}}$ & $63_{\textcolor{PineGreen}{+19}}$ & $55_{\textcolor{PineGreen}{+11}}$ & $55_{\textcolor{PineGreen}{+11}}$ & $71_{\textcolor{PineGreen}{+27}}^*$ & $55_{\textcolor{PineGreen}{+11}}$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Pythia-6.9b-chat} & No int. & $55$ & $54$ & $28$ & $36$ & $64$ & $20$ & $44$ & $67$ & $30$ \\
        & ITI & $57_{\textcolor{PineGreen}{+2}}$ & $54_{+0}$ & $28_{+0}$ & $44_{\textcolor{PineGreen}{+8}}$ & $71_{\textcolor{PineGreen}{+7}}$ & $32_{\textcolor{PineGreen}{+12}}$ & $44_{+0}$ & $67_{+0}$ & $30_{+0}^*$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $68_{\textcolor{PineGreen}{+13}}$ & $65_{\textcolor{PineGreen}{+11}}$ & $57_{\textcolor{PineGreen}{+29}}^*$ & $54_{\textcolor{PineGreen}{+18}}$ & $75_{\textcolor{PineGreen}{+11}}$ & $48_{\textcolor{PineGreen}{+28}}^*$ & $58_{\textcolor{PineGreen}{+14}}^*$ & $67_{+0}$ & $54_{\textcolor{PineGreen}{+24}}^*$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \multirow[t]{3}{*}{Pythia-12b} & No int. & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ & $44$ \\
        & ITI & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        \rowcolor{gray!20}
        \cellcolor{white}
        & CAA & $54_{\textcolor{PineGreen}{+10}}$ & $64_{\textcolor{PineGreen}{+20}}^*$ & $54_{\textcolor{PineGreen}{+10}}$ & $60_{\textcolor{PineGreen}{+16}}$ & $58_{\textcolor{PineGreen}{+14}}$ & $55_{\textcolor{PineGreen}{+11}}$ & $54_{\textcolor{PineGreen}{+10}}$ & $67_{\textcolor{PineGreen}{+23}}$ & $54_{\textcolor{PineGreen}{+10}}$ \\
        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \bottomrule
    \end{tabular}
    }
    \caption{Comparison of the effects of ITI \citep{li2023inferencetime} and CAA \citep{rimsky2023steering} activation editing methods on three tasks from BigToM \citep{gandhi2024understanding}. TB denotes a true belief task, whereas FB denotes a false belief task. The numbers represent accuracy scores, with the difference in performance compared to no intervention (No int.) indicated as subscripts (ITI $-$ No int. and CAA $-$ No int.). An asterisk ($*$) denotes a statistically significant difference from No int.\ based on a
    t-test with $p < 0.05$.}
    \label{tab:caa_results}
\end{table*}

